Random Cuts are Optimal for Explainable k-Medians

We show that the RandomCoordinateCut algorithm gives the optimal competitive ratio for explainable k-medians in l1. The problem of explainable k-medians was introduced by Dasgupta, Frost, Moshkovitz, and Rashtchian in 2020. Several groups of authors independently proposed a simple polynomial-time randomized algorithm for the problem and showed that this algorithm is O(log k loglog k) competitive. We provide a tight analysis of the algorithm and prove that its competitive ratio is upper bounded by 2ln k +2. This bound matches the Omega(log k) lower bound by Dasgupta et al (2020).

==> paper/hitting-time.tex <==
\subsection{Hitting Time and Elimination Time}

In this section, we define some useful notations for the set elimination game with the exponential clock. We first define the hitting time of any subset $X \in \Omega$ in the set elimination game.

\begin{definition}
For a subset $X \in \Omega$, the hitting time $h(X)$ of the set $X$ is defined as the first time that we sample an element from $X$,
$
h(X) = \inf \{t: \omega_t \in X\}.
$
\end{definition}

We also define the elimination time of each set $S_i$ in the set elimination game. 

\begin{definition}
Consider any set elimination game with the measure space $(\Omega,\mu)$ and $k$ sets $S_1,S_2,\dots,S_k$ in $\Omega$. For every $i\in [k]$, the elimination time $e(S_i)$ of the set $S_i$ is defined as the time when the set $S_i$ is eliminated, $e(S_i) = \inf \{t: S_i \not\in \calA_t(K)\}$. If the set $S_i$ is the winner, then $e(S_i) = \infty$.    
\end{definition}
